PaletteNeRF: Palette-based Appearance Editing of Neural Radiance Fields

Recent advances in neural radiance fields have enabled the high-fidelity 3D reconstruction of complex scenes for novel view synthesis. However, it remains underexplored how the appearance of such representations can be efficiently edited while maintaining photorealism. In this work, we present PaletteNeRF, a novel method for photorealistic appearance editing of neural radiance fields (NeRF) based on 3D color decomposition. Our method decomposes the appearance of each 3D point into a linear combination of palette-based bases (i.e., 3D segmentations defined by a group of NeRF-type functions) that are shared across the scene. While our palette-based bases are view-independent, we also predict a view-dependent function to capture the color residual (e.g., specular shading). During training, we jointly optimize the basis functions and the color palettes, and we also introduce novel regularizers to encourage the spatial coherence of the decomposition. Our method allows users to efficiently edit the appearance of the 3D scene by modifying the color palettes. We also extend our framework with compressed semantic features for semantic-aware appearance editing. We demonstrate that our technique is superior to baseline methods both quantitatively and qualitatively for appearance editing of complex real-world scenes.

==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/macros.tex <==

\usepackage{overpic}
\usepackage{enumitem} %< control spacing in itemize/enumerate/...
\usepackage{overpic} %< add raw math symbols to figures
\usepackage{color}
\usepackage{xcolor}
\usepackage{array}
\usepackage{bm}

\newcommand{\ignorethis } [1] {}
% \usepackage{microtype} %< hardcore text layout optimization (ONLY UPDATE ~DEADLINE)
% \usepackage{placeins} %< if you want to use FloatBarriers

%%
%% basic colors
%%
\definecolor{turquoise}{cmyk}{0.65,0,0.1,0.3}
\definecolor{purple}{rgb}{0.65,0,0.65}
\definecolor{dark_green}{rgb}{0, 0.5, 0}
\definecolor{orange}{rgb}{0.8, 0.6, 0.2}
\definecolor{red}{rgb}{0.8, 0.2, 0.2}
\definecolor{darkred}{rgb}{0.6, 0.1, 0.05}
\definecolor{blueish}{rgb}{0.0, 0.3, .6}
\definecolor{light_gray}{rgb}{0.7, 0.7, .7}
\definecolor{pink}{rgb}{1, 0, 1}
\definecolor{greyblue}{rgb}{0.25, 0.25, 1}

%%
%% basic TODOs
%%

\newcommand{\zhengfei}[1]{\noindent {\color{turquoise} [{\bf Zhengfei:}   {#1}]}}

\newcommand{\fujun}[1]{\noindent {\color{dark_green} [{\bf Fujun:}   {#1}]}}

\newcommand{\sai}[1]{\noindent {\color{purple} [{\bf Sai:}   {#1}]}}

\newcommand{\ZS}[1]{\noindent {\color{pink} [{\bf Zhixin:}   {#1}]}}

\definecolor{color1}{rgb}{0.36470588235, 0.7294117647, 0.43921568627}
\definecolor{color2}{rgb}{0.88235294117, 0.27450980392, 0.2431372549}
\definecolor{color3}{rgb}{0.58823529411, 0.46666666666, 0.4}
\definecolor{color4}{rgb}{0.30196078431, 0.62352941176, 0.88235294117}
\definecolor{color5}{rgb}{0.8862745098, 0.66274509803, 0.22745098039}
\newcommand{\PaletteNeRF}{{\color{color1}P\color{color2}a\color{color3}l\color{color4}e\color{color5}t\color{color5}t\color{color4}e}NeRF}

\newcommand{\comment}[1]{}

==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/abstract.tex <==
\begin{abstract}
Recent advances in neural radiance fields have enabled the high-fidelity 3D reconstruction of complex scenes for novel view synthesis. However, it remains underexplored how the appearance of such representations can be efficiently edited while maintaining photorealism. 
In this work, we present PaletteNeRF, a novel method for photorealistic appearance 
editing of neural radiance fields (NeRF) based on 3D color decomposition. 
Our method decomposes the appearance of each 3D point into a linear
combination of palette-based bases (i.e., 3D segmentations defined by a group of NeRF-type functions) that are shared across the scene. While our palette-based bases are view-independent, we also predict a view-dependent function to capture the color residual (e.g., specular shading). During training, we jointly optimize the basis functions and the color palettes, and we also introduce novel regularizers to encourage the spatial coherence of the decomposition. Our method allows users to efficiently edit the appearance of the 3D scene by modifying the color
palettes. We also extend our framework with compressed semantic features for 
semantic-aware appearance editing. We demonstrate that our technique is superior to 
baseline methods both quantitatively and qualitatively for appearance editing 
of complex real-world scenes. 

% Our implementation is available at \url{XXX}.

% In this work, we present PaletteNeRF, a new method for photorealistic appearance editing of neural radiance fields (NeRF) using soft color segmentation. Our method decomposes the scene appearance into a set of 3D-aware and view-consistent soft color palettes, each containing a layer of extracted homogeneous color region, which allows for intuitive and real-time color manipulation of 3D scenes such as recoloring, stylization and illuminance modification. 
% We project the radiance samples to normalized colorspace before palette extraction to avoid similar palettes, followed by a novel soft color decomposition approach that produces compact layers of homogeneous colors. Further, we extend our framework with compressed CLIP features for coherent and semantic-aware appearance editing. We show that our technique is superior in quality and more robust to various manipulation tasks on complex real-world scenes than baseline methods through a number of quantitative and qualitative experiments. Our implementation is available at \url{XXX}.


\end{abstract}

==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/conclusion.tex <==
\section{Conclusion}
We have presented PaletteNeRF, a novel and efficient palette-based appearance editing framework for neural radiance fields. Our method significantly increases the practicality of palette-based appearance editing and enables intuitive and controllable interactive editing on real-world scenes. Our experiments illustrate the benefit of our approach for various editing tasks such as recoloring, photorealistic style transfer and illuminance changing. Future work may include frequency-based decomposition and editing of specular highlights and extending to dynamic NeRFs.
\paragraph{Acknowledgement}
This project was in part supported by Samsung, the Stanford Institute for Human-Centered AI (HAI), and a PECASE from the ARO. We also thank Jiaman Li for helping conducting our user study.

==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/intro.tex <==
\section{Introduction}
% Neural scene representations such as Neural Radiance Fields (NeRF)~\cite{NeRF} have received increasingly more attention in recent years due to their compelling capability and robustness in representing real-world 3D scenes from 2D images for high-quality and photorealistic novel view synthesis. Although significant effort has been devoted to inventing new 3D data structures to accelerate the training and rendering of these implicit volumetric representations~\cite{PlenOxels, Instant-NGP, KiloNeRF, TensoRF}, it still remains challenging and underexplored regarding how to efficiently edit these representations for 3D content re-creation and photorealistic manipulation in an intuitive and controllable manner. In particular, it is non-trivial to perform local image manipulations on 2D views that can be efficiently propagated to NeRF scene appearance while maintaining 3D consistency and photorealism, especially for complex real-world scenes.  

Neural Radiance Fields (NeRF)~\cite{NeRF} and its variants
~\cite{PlenOxels, Instant-NGP, KiloNeRF, TensoRF} have received
increasing attention in recent years for their ability to robustly reconstruct real-world 3D scenes from 2D images and enable high-quality, photorealistic novel view synthesis.
%While such volumetric representations have great advantages in representing highly complex scenes, 
However, such volumetric representations are challenging to edit due to the fact that scene appearance is implicitly encoded in neural features and network weights that do not support local manipulation or intuitive modification.  

Multiple approaches have been proposed to support editing of NeRF. One category 
of methods~\cite{NeRFactor,NeROIC,NeRD,PhySG} recover the material properties of the scene so that they can re-render them under novel lighting conditions or adjust the material properties
such as surface roughness. Such methods rely on accurate estimation of the 
scene reflectance, which is typically challenging for 
real-world complex scenes captured under unconstrained environment. Another category of
methods~\cite{CLIP-NeRF,NeRF-W} learns a latent code on which NeRF can be conditioned to produce the desired  
appearance. However, these methods often suffer from limited capacity and flexibility and do 
not support fine-grained editing. In addition, some other methods~\cite{ARF} learn to transfer the appearance of NeRF to match a given style image, but sometimes
fail to maintain the same level of photorealism in the original scene.


In this paper, we propose \emph{\PaletteNeRF}, a novel method to 
support flexible and intuitive editing of NeRF. Our method is inspired by 
previous image-editing methods based on color 
palettes~\cite{chang2015palette, RGBXY}, where a small 
set of colors are used to represent the full range of colors in the image.  
We model the radiance of each point using a combination 
of specular and diffuse components, and we further decompose the
diffuse component into a linear combination of view-independent color bases 
that are shared across the scene.
During training, we jointly optimize the per-point specular component, the global color bases and the per-point linear weights to minimize the difference between the rendered images and the ground truth images. We also introduce novel regularizers 
on the weights to encourage the sparseness and spatially coherence of the decomposition and 
achieve more meaningful grouping. With the proposed framework, we can intuitively 
edit the appearance of NeRF by freely modifying the learned color 
bases (Fig.~\ref{fig:teaser}). We further show that our framework can be combined with 
semantic features to support semantic-aware editing. Unlike previous palette-based image~\cite{RGBXY, FSCS} or video~\cite{du2021video} editing methods, our method produces more globally coherent and 3D consistent recoloring results of the scene across arbitrary views. We demonstrate that our method can enable more fine-grained local color 
editing while faithfully maintaining the photorealism of the 3D scene, and 
achieves better performance than baseline methods both quantitatively and qualitatively. In summary, our
contributions include:

% Existing approaches that tackle the appearance editing problem of NeRF can be classified into mainly two categories --- material-based models~\cite{NeRFactor, NeROIC, NeRD, PhySG} and embedding-based models~\cite{CLIP-NeRF, NeRF-W, ARF}. Material-based models typically condition NeRF appearance on physical light transport and try to solve for BRDF materials, geometry and illumination in a joint inverse rendering optimization procedure. While this type of methods allow us to generate high-quality, controllable 3D assets that suit well the traditional computer graphics pipelines (e.g., Unreal Engine~\cite{sanders2016introduction}), all physical parameters are required as input and therefore it is prone to error for real-world data where the surrounding illumination, materials and geometry occlusions can be arbitrarily complex. As a result, these methods are often limited to object-level 3D capture with rather simplified rendering models. On the other hand, embedding-based models address this problem through latent appearance modeling. Specifically, a latent embedding space~\cite{NeRF-W} is introduced to explain and control NeRF's scene appearance from capturing variations such as time-varying illumination and photometric post-processing. Unlike the material-based models, embedding-based approaches are often more robust to complex real-world scenes and are able to model NeRF's appearance variations reasonably. Unfortunately, these embedding-based models tend to suffer from limited capacity in appearance manipulation and are often less intuitive to edit, since it is difficult to interpret or control in the embedded latent space from a physical viewpoint. Therefore, there is an emerging interest in balancing the trade-off between these two categories, i.e., offering an intuitive appearance editing mode suitable for neural scene representations with improved robustness in handling real-world scenes. 

% In this paper, we propose \emph{PaletteNeRF}, a novel and efficient method of appearance decomposition, to help us explore new ways of editing on NeRF. Inspired by the color palette techniques in image editing~\cite{DBLP:journals/tog/Finkelstein15, RGBXY}, we introduce a set of 3D-aware, view-consistent soft color segmentation layers, each containing a layer of extracted homogeneous color region, that compactly represent the different components of the captured scene appearance. We further incorportate compressed CLIP features to improve its performance in handling semantic-aware editing. As a result, we show that PaletteNeRF can be robustly applied to different appearance editing tasks, such as recoloring, example-based stylization and illuminance changing. In summary, our main contributions include:

\begin{itemize}
% \item We propose a novel and general appearance editing framework for NeRF  % decomposed into a set of 3D-aware, view-consistent soft color segmentation layers. 
\item We propose a novel framework to facilitate the editing of NeRF by decomposing the radiance field into a weighted combination of learned color bases.

\item We introduced a robust optimization scheme with novel regularizers to achieve intuitive decompositions.

\item Our approach enables practical palette-based appearance editing, making it possible for novice users to interactively edit NeRF in an intuitive and controllable manner on commodity hardware.

% \item We design a robust and efficient palette-based optimization pipeline and further incorporate compressed CLIP features for semantic-aware appearance editing. 

% \item Our approach significantly increases the practicality of palette-based appearance editing, making it possible for average users to edit NeRF in an intuitive and controllable manner on a commodity computer interactively.
\end{itemize}
 






==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/method.tex <==

\section{Method}

% \section{Method} 
% Given a set of multi-view images of a scene, our goal is to achieve high quality and view consistent appearance editing on the scene, for example, color changing and highlight enhancing. To do this, we first introduce a general NeRF-based method by introducing neural basis functions. Each neural basis function represents a specific view-dependent shading effect of the appearance. We then design two models from this general method. The first model aims to extract color palettes with radiance bases of the scene, and the second model decomposes shadings components at different frequency domains. 
\begin{figure*}
\centering
\includegraphics[width=1.0\linewidth]{figures/overview.pdf}
\vspace{-20px}
\caption{\textbf{The overview of our pipeline}. Given a set of training images, we first (a) reconstruct the scene geometry and build the color palettes with existing methods. Then, our \PaletteNeRF{} (b) decomposes the scene appearance into multiple palette-based bases and the view-dependent color. We deploy a series of losses on the palette-based base's functions, the view-dependent color, and the final output. }
\label{fig:overview}
\end{figure*}

Fig.~\ref{fig:overview} illustrates the overview of our multi-stage pipeline.  Given a set of images with known poses from a scene, we first optimize a NeRF-based model to reconstruct the geometry of the scene. Then, we extract $N_p$ color palettes with the input images and the learned scene geometry. Finally, we train a segmentation model to decompose the scene appearance into multiple bases based on the extracted palettes. Our decomposition result is able to drive various downstream applications, such as recoloring, photorealistic style transfer and illuminance modification. 

\subsection{Volumetric Rendering}
We build our model on the widely used framework Neural Radiance Fields (NeRF). Typically, a NeRF-based model optimizes two neural functions: a geometry function $\sigma(\bm{x})$ and a color function $\bm{c}(\bm{x}, \bm{d})$. The geometry function takes a 3D position as input and outputs the density at this point. The color function takes a 3D position and a viewing direction as input and output a corresponding RGB color.
To render an image from a given camera pose, NeRF samples batches of rays from the camera to render the pixels. For each sampled ray $\bm{r} = (\bm{o}, \bm{d})$, a group of 3D points are sampled along the ray path $\bm{x}_{1..M}$ with depth $t_{1..M}$, where $\bm{x}_i = \bm{o} + t_i \bm{d}$. The color prediction of the ray $\bm{r}$ is calculated as:
\begin{equation}
    \bm{c}(\bm{r})=\sum_{i=1}^{M}\alpha_i(1-w_i)\bm{c}(\bm{x}_i, \bm{d}),
    \label{eq:NeRF}
\end{equation}
where 
$w_i=\exp(-(t_i-t_{i-1})\sigma(\bm{x}_i))$ is the transmittance of the ray between the $i$'th sample point and the $(i+1)$'th sample point, and $\alpha_i=\prod_{j=1}^{i-1}w_i$ is the ray attenuation from the ray's origin to the $i$'th sample point. 

\begin{figure}
\centering
\includegraphics[width=0.495\textwidth]{figures/palette_extraction.pdf}
\caption{\textit{Left:} Reference image; \textit{Middle:} Comparison between the recoloring result of our model trained with extracted palettes and model trained with random initialized palettes; \textit{Right:} Normalized training image and the extracted palettes from normalization of different levels.}
\label{fig:palette_extraction}
\end{figure}

\subsection{Palette Extraction}
Although it is possible to directly train our model with randomly initialized color palettes, doing this will bring excessive ambiguity to the problem and may produces irregular results as shown in Fig.~\ref{fig:palette_extraction}(b). Thankfully, the problem of extracting color palettes from images has been extensively researched over the past years, thus we use the extraction method from a state-of-the-art image recoloring work~\cite{RGBXY} as our initialization. In general, this method extracts color palettes from the 3D convex hull of the clustered image colors in the RGB space.
% \comment{this method first groups the RGB image colors using the K-means clustering algorithm with a relatively large cluster number, then calculate the 3D convex hull of the cluster centers. The convex hull is further simplified by a greedy-based edge collapsing algorithm, and the vertices of the remaining geometry is the output.}
In our scenario, we simply select all training image pixels with valid depth from NeRF's depth maps and concatenate their color as input.

We notice that with input from multiple images, the extraction method may produce palettes that are chromatically similar (e.g., palettes including a light yellow and a dark yellow), due to the varying shading of the captured scene. This may result in unrealistic appearance editing. Inspired by image illumination decomposition works~\cite{carroll2011illumination, Meka:2021}, we normalize the input colors of the training images by their intensity, to narrow down the search space of color palettes. Conventionally, the intensity of a color is represented by the L1 norm of its RGB value. However, normalizing with L1 norm projects the colors to a plane, which is a highly ill-posed edge case for 3D convex hull calculation. These problems can be addressed by replacing the norm with a higher order one. Empirically, we find that palettes extracted from L2 normalized images work well in our next decomposition stage, and use them in all of our experiments.

In addition to the extracted palettes $\bar{\bm{\mathcal{P}}}$, we also keep the blending weights $\bar\omega$ of the input pixel colors, calculated from the method of the same work. These weights act as an additional supervision in the next stage.

\subsection{Color Decomposition}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/network.pdf}
\caption{\textbf{Our network structure.} As we only show one palette-based basis in the figure, our network generates $N_p$ bases in parallel and they are summed up in the final step.}
\label{fig:basis_segmentation}
\end{figure}

To introduce our color decomposition model, we first explain our target outputs, then describe the structure of our decomposition network. 

%The overview of our framework is shown in Fig.~\ref{fig:overview}. 
As shown in Fig.~\ref{fig:overview}, given the color palettes of size $N_p$, our model aims to reconstruct $N_p$ view-independent palette-based bases and an additional view-dependent color function representing all view-dependent shading such as specular reflections. The palette-based bases correspond to the extracted color palettes, and are defined by two functions of $\bm{x}$: A color offset function $\bm{\delta}: \mathbb{R}^3 \rightarrow \mathbb{R}^3$, and a weight function $\omega: \mathbb{R}^3 \rightarrow [0,1]$. Observing that realistic image captures usually consists of a huge variety of colors, we allow the basis color of each point shift from the palette color with an offset (inspired by image-based soft color segmentation methods ~\cite{aksoy2017unmixing, FSCS}). This design increases the capacity of the bases and benefits the segmentation quality on complex scenes. We also introduce an intensity function $I: \mathbb{R}^3 \rightarrow [0,1]$ that is shared among all palette-based bases, due to the normalization of the extracted palettes. While the aforementioned functions only take position as input, our model also contains a view-dependent color function $\bm{s}: \mathbb{R}^5 \rightarrow [0,1]^3$ that takes viewing direction as input, too. We compose all of these bases into a color output $\bm{c}\in \mathbb{R}^3$ by the following equation:
\begin{equation}
\bm{c}(\bm{x}, \bm{d}) = \bm{s}(\bm{x}, \bm{d}) + I(\bm{x}) \sum_{i=1}^{N_p} \omega_i(\bm{x}) \left(\bm{\mathcal{P}}_i + \bm{\delta}_i(\bm{x})\right),
\label{eq:color_segmentation}
\end{equation}
where $\omega_i(\bm{x})$ are normalized by their sum. We clamp the summed-up color $\bm{c}$ to $[0, 1]$ as the final output. We also optimize the palette color $\bm{\mathcal{P}}_i$ during the training. As shown in Fig.~\ref{fig:basis_segmentation}, Our network consists of three MLPs: the Diffuse MLP predicts the diffuse color $\bm{c}_d(\bm{x})$, i.e. the sum of all palette-based bases; the View-Dependent MLP generates view-dependent color $\bm{s}(\bm{x}, \bm{d})$; Finally, the Palette MLP predicts the function values of the palette-based bases: $\omega_i(\bm{x}), \bm{\delta_i}(\bm{x})$ and $I(\bm{x})$, where $\bm{c}_d$ is also fed as an input prior. We compose all of the network outputs to the final color using Eq.~\ref{eq:color_segmentation}.

\subsection{Optimization}

Given the fact that separating multiple bases from the scene appearance is a considerably ill-posed task, a lot of cautions should be taken in designing the optimization scheme. Hence, we develop a series of losses to regulate the optimized parameters and to avoid undesirable results such as local-minimum. 

To begin with, we deploy the image reconstruction loss defined as:
\begin{equation}
\mathcal{L}_{
\textrm{recon}} = \lVert \bm{c}^{\textrm{ref}} - \bm{c}(\bm{r})\rVert _2^2 + \lVert \bm{c}^{\textrm{ref}} - \left(\bm{c}_d(\bm{r})+\bm{s}(\bm{r})\right)\rVert _2^2,
\label{eq:img_loss}
\end{equation}
where $\bm{c}^{\textrm{ref}}$ is the ground truth color, $\bm{c}(\bm{r}), \bm{c}_d(\bm{r}), \bm{s}(\bm{r})$ are calculated from the volume rendering equation at Eq.~\ref{eq:NeRF}. The second term of this loss can also be considered as the L2 distance between $\bm{c}_d(\bm{r})$ and the sum of palette-based bases. 
We also add a regularization loss $\mathcal{L}_\textrm{s}$ to the view-dependent color function $\bm{s}(\bm{x}, \bm{r})$, to prevent the particular situation where $\bm{s}$ dominates the appearance and pushes all palette-based bases to 0. This loss is defined as:
\begin{equation}
\mathcal{L}_\textrm{s} = \lVert \bm{s}(\bm{x}, \bm{d}) \rVert _2^2.
\label{eq:s_loss}
\end{equation}

While our model uses color offsets to shift the basis color, it is necessary to restrict the blending weights and color offset to avoid extreme solutions. Hence, we adapt the sparsity loss $\mathcal{L}_{\textrm{sp}}$ and the color offset loss $\mathcal{L}_{\textrm{offset}}$ from the image soft segmentation method \cite{aksoy2017unmixing} . They are defined as: 
\begin{align}
\mathcal{L}_{\textrm{sp}} &= \frac{\sum_{i=1}^{N_p} \omega_i(\bm{x})}{\sum_{i=1}^{N_p} \omega_i^2(\bm{x})} - 1,
\label{eq:sparse_loss} \\
\mathcal{L}_{\textrm{offset}} &= \lVert \bm{\delta}(\bm{x}) \rVert _2^2.
\label{eq:offset_loss}
\end{align}
The sparsity loss aims to make the blending weights sparser (e.g., segmenting each point $\bm{x}$ to fewer bases), which will eventually increase the capacity of the bases by increasing the color offset. On the other hand, the color offset loss directly suppresses the magnitude of color offsets, preventing them from deviating from the palettes too much. Intuitively, these two losses act as two adversarial roles, and finding a good balance between them will lead to neat segmentation results with reasonable basis color. In our experiments, however, we observe that these two losses may lead to harsh segmentation results, which will drastically affect the quality of the following editing (see our qualitative ablation study). Thus we introduce a novel 3D-aware smooth loss to smooth the weight function based on the NeRF's output. It is given by:
\begin{equation}
\mathcal{L}_{\textrm{sm}} = \xi(\bm{x}, \bm{x}+\bm{\varepsilon}) \lVert \bm{\omega}(\bm{x}) - \bm{\omega}(\bm{x}+\varepsilon) \rVert ^2,
\label{eq:delta_loss}
\end{equation}
where $\bm{\omega}=\omega_{1...N_p}, \bm{\varepsilon}$ is a random position offset sampled from a Gaussian distribution, and $\xi(\cdot)$ is the similarity between two points. Here, we adapt the Gaussian kernel used in the bilateral filter, and define the similarity function as:
\begin{equation}
\xi(\bm{x}, \bm{y}) = \exp(-\frac{\lVert\bm{x} - \bm{y}\rVert^2}{\sigma_x} - \frac{\lVert \bm{c}_d(\bm{x}) - \bm{c}_d(\bm{y})\rVert^2}{\sigma_c}),
\label{eq:delta_loss}
\end{equation}
where $\sigma_x$ and $\sigma_c$ are smoothing parameters. While the diffuse color $\bm{c}_d$ is used in the smooth loss, we cut off their gradients during the training. 
%In Sec.~\ref{sec:results}, we will show in an ablative way how the sparsity loss, color offset regularization loss and smooth loss will improve our final outputs.

Finally, we add two more losses that incorporate the supervisions from the palette extraction model. They are:
\begin{align}
\mathcal{L}_{\textrm{palette}} &= \lVert \bm{\mathcal{P}} - \bar{\bm{\mathcal{P}}} \rVert _2^2, \\
\mathcal{L}_{\textrm{weight}} &= \lVert \omega - \bar{\omega} \rVert _2^2.
\label{eq:palette_loss}
\end{align}
As a summary, the overall loss of our optimization is the weighted sum defined as:
\begin{equation}
    \begin{split}
    \mathcal{L} &= \mathcal{L}_\textrm{recon} 
    + \lambda_\textrm{s} \mathcal{L}_\textrm{s} 
    + \lambda_{\textrm{sp}} \mathcal{L}_{\textrm{sp}} \\
    & + \lambda_{\textrm{offset}} \mathcal{L}_{\textrm{offset}} 
    + \lambda_{\textrm{sm}} \mathcal{L}_{\textrm{sm}} \\
    & + \lambda_{\textrm{palette}} \mathcal{L}_{\textrm{palette}}
    + \lambda_{\textrm{weight}} \mathcal{L}_{\textrm{weight}},
    \label{eq:overall_loss}
    \end{split}
\end{equation}
where $\lambda_\textrm{s}, \lambda_{\textrm{sp}}, \lambda_{\textrm{offset}}, \lambda_{\textrm{sm}}, \lambda_{\textrm{palette}}, \lambda_{\textrm{weight}}$ are all loss weights. 

\subsection{Appearance Editing}

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth, height=0.5\linewidth]{figures/holder.png}
% \caption{Appearance Editing}
% \label{fig:appearance_editing}
% \end{figure}

With the bases predicted from the model, we can simply tune the value of the functions to support appearance editing, such as recoloring and photorealistic style transfer. When deployed with recent fast NeRF models, our method is able to achieve real-time interactive editing. We will further explain the editing details in the next section.

Since our basis functions are defined on the whole scene, they do not directly support local editing (e.g., edit a single object in the scene). To achieve that, we follow one recent work~\cite{DBLP:journals/corr/abs-2205-15585} that learns a 3D feature field from the semantic feature maps predicted from state-of-the-art image-based segmentation models (e.g., Lang-Seg~\cite{DBLP:conf/iclr/LiWBKR22}), and use the feature field to guide the editing. However, directly adding high dimensional semantic features to our model may decrease its efficiency, making it impractical to edit in real-time. As the objects captured from a scene are often limited to a small set (e.g., in an indoor scene, chairs, walls and floor are the most likely appeared objects),  the  semantic features extracted from the scene are often a limited subset of the whole feature space. Therefore, we apply PCA to compress the extracted features to a lower dimension (16 in our experiments) before feeding them to the network.~\footnote{Please find more details in terms of implementation, usage and results on semantic guided editing in the supplemental materials.} 
% \comment{We will show in the experiments that this technique significantly shorten the inference time and does not noticeably affect the editing quality.}

% % <Introduction of NeRF>
% \subsection{Neural Radiance Field} 
% The original NeRF model consists of two MLPs: a geometry MLP denoted as $f_\sigma(\textbf{x})$ and a color MLP $f_c(\textbf{x}, \textbf{r})$. The geometry MLP takes the position of a 3D point as input and outputs the density at this point. The color MLP takes the position and viewing direction of a 3D point and output its RGB color.

% Given a set of input images $I_{1...N_k}$, with their respective camera parameters $P_{1...N_k}$, NeRF samples batches of randomly sampled rays from the cameras to train its model. For each ray $\bm{r} = (\bm{o}, \bm{d})$ sampled from $P$, a group of 3D points are sampled along the ray path $\bm{x}_{1..N_p}$ by depth values $t_{1..N_p}$, where $\bm{x}_i = \bm{o} + t_i \bm{d}$. The color prediction or the ray $\bm{r}$ is  defined as:
% \begin{equation}
%     C(\bm{r})=\sum_{i=1}^{N_p}\alpha_i(1-w_i)f_c(\bm{x}_i, \bm{d}),
%     \label{eq:NeRF}
% \end{equation}
% where 
% $w_i=\exp(-(t_i-t_{i-1})f_\sigma(\bm{x}_i))$ is the transmittance of the ray between the $i$'th sample point and the $(i+1)$'th sample point, and $\alpha_i=\prod_{j=1}^{i-1}w_i$ is the ray attenuation from the ray's origin to the $i$'th sample point. Moreover, NeRF applies the widely used Sinusoidal Positional Embedding to encode $\bm{x}$ and $\bm{d}$ as the input of the MLPs. NeRF uses the reconstruction error between the predicted ray color $C(\bm{r})$ and the ground truth color from the input images as the supervision.

% % <Definition of the neural basis decomposition>
% \subsection{Neural Basis Decomposition}
% Since the original NeRF model predicts the output color from only a single source (i.e., the color MLP), it is not able to decompose the appearance of the captured scene into different parts, which are essential for many downstream editing applications, for example, changing the color of an object appeared in the scene while keeping the other part unchanged. We thus introduce Neural Basis Decomposition to achieve this goal. We replace the color prediction of NeRF with the weighted sum of multiple color outputs. Specifically:
% \begin{equation}
% f_c(\bm{x}, \bm{d}) = \sum_{i=1}^{N_b} B(\phi_i(\bm{x}, \bm{d}, \theta_i), \theta_i)p_i(\bm{x})
% \end{equation}
% where $p_i(\bm{x})$ is the blending weight of the $i$'th basis at the 3D point $\bm{x}$, and $B(\phi_i(\bm{x}, \bm{d}, \theta_i), \theta_i)$ is the neural basis function. The neural basis function has two parameters: a global parameter $\theta$, which represents the fundamental properties of the basis (for example, the colors of the color palette), and a function $\phi(\bm{x}, \bm{d}, \theta_i)$, which represents the influence of basis $B$ at a certain 3D point. The other rendering equations of our model are the same as the equations in NeRF. Next, we present two models of the Neural Basis Decomposition method: a color-palette-based model and a frequency-based model.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{figures/patent/color_palette.png}
% \end{center}
% \vspace{-10px}
% \caption{
% \textbf{Network architecture of our color palette model.} }
% \vspace{-5pt}
% \label{fig:color_palette_model}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{figures/patent/color_palette_result.png}
% \end{center}
% \vspace{-10px}
% \caption{
% \textbf{Result of our color palette model.} \textit{Up}: the original output of the model (without color changes); \textit{Down}: Results with edited color. }
% \vspace{-5pt}
% \label{fig:color_palette_result}
% \end{figure}

% \subsection{Color Palette Model}
% In our color palette model, the global property of each basis $\theta i$ is defined as an RGB value $c_i$, and the $\phi$ function is an MLP predicting monochromatic radiance value $r_i$. The neural basis function $B$ is simply the product of $c_i$ and $r_i$. As shown in Fig. \ref{fig:color_palette_model}, we train two MLPs to predict $p_i$ and $r_i$ given inputs of a 3D point and optimize $c_i$ as global parameters. The output color $C$ is the sum of the colors of each basis, which is the product of $p_i, r_i, c_i$ together.

% We show the results of our color palette model on two datasets. The first one is the Lego scene from the NeRF's datasets, and we changed the yellow part of the model to purple; the second is a scene we rendered ourselves: a Kitti model placed on a glossy plane. In this case, We change the pink part of the Kitti into cyan. Results are shown in Fig. \ref{fig:color_palette_result}.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{figures/patent/frequency.png}
% \end{center}
% \vspace{-10px}
% \caption{
% \textbf{Network architecture of our frequency-based model.} }
% \vspace{-5pt}
% \label{fig:frequency_model}
% \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{figures/patent/frequency_result.png}
% \end{center}
% \vspace{-10px}
% \caption{
% \textbf{Result of our frequency-based model.} We show three basis outputs with different theta values from two different views. Notice that the high-frequency basis produces a varying reflection on the plane between different views while the other two generate a static reflection. }
% \vspace{-5pt}
% \label{fig:frequency_result}
% \end{figure}

% \subsection{Frequency-based Decomposition Model}
% We also apply our Neural Basis Decomposition method to decompose the scene appearance into different shading terms, for example, diffuse and specular terms. In this case, each neural basis represents a shading component for a specific frequency domain. The higher the frequency is, the glossier the shading effect should be. Specifically, we control the frequency domain of a neural basis by adding the basis property $\theta$ to the Sinusoidal Positional Embedding of the viewing direction $\bm{r}$. We change the embedding from
% \begin{equation}
% z(\bm{r}) = \{\mathrm{sin}(2^d\bm{r}), \mathrm{cos}(2^d\bm{r}), d\in 0...D \}
% \label{eq:original_PE}
% \end{equation}
% to
% \begin{equation}
% z_i(\bm{r}) = \{\mathrm{sin}(2^d\bm{r})*\theta_i^d, \mathrm{cos}(2^d\bm{r})*\theta_i^d, d\in 0...D \}
% \label{eq:new_PE}
% \end{equation}
% where $\theta_i$ becomes a scalar parameter between 0 to 1. $\phi_i$ is set to the NeRF's color MLP with the updated position embedding, and $B$ becomes the identity function. Fig. \ref{fig:frequency_model} shows the network structure of this model, and Fig. \ref{fig:frequency_result} shows one of the results of this model.


% % Many follow-ups, such as NeRFactor\cite{NeRFactor}, PhySG\cite{PhySG} and NeROIC\cite{NeROIC}, apply existing physically-based rendering methods to the NeRF to decompose the appearance into physically meaningful parts, such as environment lighting map, diffuse albedo, and BRDF parameters. 

% % <Our color-palette formulation>




==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/related.tex <==
\section{Related Work}

% \paragraph{Neural fields for rendering.}
% The emergence of neural rendering methods has greatly impacted the industry and society over recent years. Among them, many popular methods are based on neural fields \cite{PIFu, DeepSDF, VolSDF, NeuS, NeRF}. Typically, these methods use neural networks to build 3D fields that represent the geometry and appearance of the scene. While being able to render novel views with high quality, these methods usually require high time costs for training and inferring. Many recent works attempt to speed up the model by applying advanced data structures \cite{PlenOctrees, PlenOxels, TensoRF, Point-NeRF} to optimize the network structure \cite{KiloNeRF, R2L}, some can reduce the time costs to seconds \cite{PlenOxels, Instant-NGP}. These methods are designed to synthesize novel views with an appearance consistent with the input images and do not support appearance editing.

\paragraph{Neural radiance fields.}
Neural radiance fields in the form of MLPs have been extensively used for neural 
rendering tasks such as novel view synthesis.  Typically, these methods 
\cite{VolSDF, NeuS, NeRF,sitzmann2019srns} encode the geometry and appearance 
of the scene into network weights of the MLPs. Many recent works 
~\cite{PlenOxels, TensoRF, Point-NeRF, zhang2022nerfusion, Instant-NGP} propose
to speed up the training and improve the performance of the models by applying 
a combination of light-weight MLPs and neural feature maps or volumes. 
However, different from traditional graphics primitives such as triangle meshes,
both the neural features and the network weights represent scene appearance
in an implicit manner and do not support intuitive editing or controls such as recoloring, thereby greatly limiting their applications in existing graphics pipelines.  


% \paragraph{Appearance editing on NeRF.}
% One of the most representative neural field methods is NeRF\cite{NeRF}. It is based on the volume rendering technique, and consists of two multi-layer perceptrons (MLP) to predict the geometry and color of the scene given input coordinates.  Following the success of NeRF, many works further explore how to edit the color output of NeRF. One standard solution is to decompose physically based materials from the environment, which can be either consistent \cite{NeRFactor, NeRV, Ref-NeRF} or different \cite{NeRV, NeRD, Neural-PIL, NeROIC, SAMURAI, NeRS} between the training images. A recent work \cite{DBLP:journals/corr/abs-2204-06837} takes indirect illuminations into account to generate more accurate materials. All these works are built on the framework of physically based rendering. Thus, they are limited to certain types of editing, such as relighting and material editing. Another group of works \cite{NeRF-W, CLIP-NeRF, AE-NeRF} try to use embedding vectors to control the appearance output. In addition to the original reconstruction loss in NeRF, adversarial losses \cite{GRAF, GIRAFFE, pi-GAN, EG3D} and perceptual losses \cite{ARF, StyleNeRF} are also used in this type of method to produce better editing results. However, these methods rely on additional sources, e.g., texts or reference images, to control the editing, thus being vulnerable to unintended editing and artifacts. Our model is robust to all the above issues, supporting flexible and explicit appearance editing.

% \paragraph{Appearance editing on NeRF.}
% One of the most representative neural field methods is NeRF\cite{NeRF}. It is based on the volume rendering technique, and consists of two multi-layer perceptrons (MLP) to predict the geometry and color of the scene given input coordinates.  Following the success of NeRF, many works further explore how to edit the color output of NeRF. One standard solution is to decompose physically based materials from the environment, which can be either consistent \cite{NeRFactor, NeRV, Ref-NeRF} or different \cite{NeRV, NeRD, Neural-PIL, NeROIC, SAMURAI, NeRS} between the training images. A recent work \cite{DBLP:journals/corr/abs-2204-06837} takes indirect illuminations into account to generate more accurate materials. All these works are built on the framework of physically based rendering. Thus, they are limited to certain types of editing, such as relighting and material editing. Another group of works \cite{NeRF-W, CLIP-NeRF, AE-NeRF} try to use embedding vectors to control the appearance output. In addition to the original reconstruction loss in NeRF, adversarial losses \cite{GRAF, GIRAFFE, pi-GAN, EG3D} and perceptual losses \cite{ARF, StyleNeRF} are also used in this type of method to produce better editing results. However, these methods rely on additional sources, e.g., texts or reference images, to control the editing, thus being vulnerable to unintended editing and artifacts. Our model is robust to all the above issues, supporting flexible and explicit appearance editing.

\paragraph{Appearance editing with NeRF.} 
Many methods have been proposed to support appearance editing of NeRF. 
Some methods~\cite{NeRFactor, NeRV, NeRD, Neural-PIL} recover the physical 
properties of the scene such as albedo, specular roughness, and then they 
can support rendering the scene under novel lighting conditions or changing  
its material properties. Some other works~\cite{NeRF-W, CLIP-NeRF, AE-NeRF}
learn a latent code jointly with the NeRF reconstruction so as to control 
its appearance such as changing the illuminations or colors by taking
new latent codes as input, which can be mapped from user input or interpolated 
from existing latent codes. Moreover, there are also approaches~\cite{ARF, StyleNeRF, UPST-NeRF} that try to 
optimize the NeRF to match its appearance against the provided 
style images. All these methods do not support fine-grained intuitive color 
editing of NeRF as ours. Concurrently, Ye et al.~\cite{ye2022intrinsicnerf} introduces a NeRF-based intrinsic decomposition model which enables 3D intuitive recoloring, but it does not support palette-based editing.


% \paragraph{Palette-based recoloring methods.}
% A number of palette-based image recoloring methods\cite{chang2015palette,DBLP:conf/siggrapha/FurusawaHOO17,DBLP:journals/tip/ZhangXST17,DBLP:journals/tog/ZouMGDF19} aim to decompose the input image into a set of monochromatic image components with different intrinsic colors (i.e., color palette), then recolor the image by modifying the intrinsic colors. \cite{DBLP:journals/tog/TanLG17,RGBXY} efficiently decompose the intrinsic colors with the geometry distribution of pixels in the RGB space. \cite{DBLP:journals/tog/CarrollRA11} incorporates the radiance transfer function and is able to decompose different shading effects. These methods are designed for image editing only and are unaware of any 3D information. On the other hand, NeRF-based decomposition methods~\cite{DBLP:journals/cgf/TojoU22, ye2022intrinsicnerf} exploit 3D information to better factorize the scene into the spatially and temporally consistent components. Similarly, our model takes multi-view images as input; thus, it can integrate the information from different views to extract globally coherent and reasonable intrinsic colors, which produces view-consistent and 3D-aware appearance editing results. 

\paragraph{Palette-based editing.}
Color palette-based 
methods~\cite{chang2015palette,DBLP:conf/siggrapha/FurusawaHOO17,DBLP:journals/tip/ZhangXST17,DBLP:journals/tog/ZouMGDF19,DBLP:journals/tog/TanLG17,RGBXY}
have been previously used in 2D image editing tasks such as recoloring. 
However, it is non-trivial to  adapt such methods for NeRF editing and  
naively performing the editing on each rendered frame cannot guarantee 
view-consistent results. Instead, we integrate the learning of the color bases 
and the spatially varying weights into the NeRF optimization process, 
thereby enabling view-consistent and 3D-aware editing. A recent work~\cite{DBLP:journals/cgf/TojoU22} proposes a palette-based recoloring method on NeRF with posterization. However, it is limited to non-photorealistic editing only.
% \sai{The last sentence does not seem to be correct.}


==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/results.tex <==




\section{Results}
\label{sec:results}

\subsection{Implementation details}
\paragraph{Training.} 
To support real-time appearance editing, we use Instant-NGP~\cite{Instant-NGP} as our backbone. \comment{Instant-NGP is a grid-based NeRF model that uses a feature hashing table to represent the 3D feature grid of the scene, which is used as the input position embeddings. It supports instant-level view synthesis in an interactive interface.}For the geometry learning stage, we keep all original configurations, except adding a per-point rgb loss introduced by Sun et al.~\cite{DVGO} to make the density field sparser and avoid floaters. For the segmentation learning stage, we fix the extracted palettes for the first 100 epochs. After that, we unleash the palettes and  remove $\mathcal{L}_{\textrm{weight}}$ to fine-tune the model. Moreover, since our smooth loss $\mathcal{L}_{\textrm{sm}}$ employs the diffuse color $\bm{c}_d$ to calculate the smoothing weight, we do not apply $\mathcal{L}_{\textrm{sm}}$ for the first 30 epoches to avoid unconverged $\bm{c}_d$ as input.

Our training and testing experiments are implemented using PyTorch~\cite{PyTorch}, and run on a single NVIDIA RTX 3090 GPU. For both stages, we train our model for 300-600 epochs (depending on the number of training images) using the Adam Optimizer~\cite{Adam} with learning rate set to $0.01$, which takes no more than 2 hours in total.

\paragraph{Datasets.} 
We conduct experiments on scenes from three sources: Lego, Ficus, Ship and Hotdog from the NeRF Blender dataset~\cite{NeRF}, Fern, Horns, Flower, Orchids from the the forward-facing LLFF dataset~\cite{LLFF} and Bonsai, Kitchen and Room from the 360-degree Mip-NeRF360 dataset~\cite{Mip-NeRF360}. 
%11 scenes from the three datasets are selected: in the Blender Dataset;  in the LLFF Dataset;  in the Mip-NeRF360 Dataset. 

\subsection{Comparisons}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/experiment/0_posternerf.pdf}
\vspace{-10px}
\caption{\textbf{Qualitative comparison with PosterNeRF}~\cite{DBLP:journals/cgf/TojoU22}. Since PosterNeRF uses more palettes, we also show their results with edits on multiple palettes for fair comparison. Zoom in for details.}
\label{fig:posterNeRF}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/experiment/7_video.pdf}
\caption{\textbf{Qualitative comparison with video palette-based recoloring method}~\cite{Du:2021:VRS}. Unlike Du et al.~\cite{Du:2021:VRS} that either only modifies the lego color (Edit 1) or introduces view-inconsistency when also modifying the gloves (Edit 2), our method recolors the 3D scene consistently while maintaining photorealisim across views. }
\label{fig:video_recolor}
\vspace{-5px}
\end{figure}

\begin{figure*}
\centering
\includegraphics[width=0.99\textwidth]{figures/experiment/1_recolor_v2.pdf}
\caption{\textbf{Qualitative comparison with image palette-based recoloring methods}. We compare our method with Tan et al.~\cite{RGBXY} and Akimoto et al.~\cite{FSCS}. For each recolored image, we also show the corresponding palettes editing on its left side, and a zoom-in view on its right side.}
\label{fig:recolor}
\vspace{-5px}
\end{figure*}

\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures/experiment/3_userstudy.pdf}
\caption{\textbf{User study results.} For each comparison we demonstrate the percentage of users who prefer our method, users who prefer the baseline method, and users who do not lean towards anyone.}
\label{fig:user_study}
\vspace{-5px}
\end{figure} 

\begin{figure*}
\centering
\includegraphics[width=1.\textwidth]{figures/experiment/2_stylization.pdf}
\caption{\textbf{Qualitative comparison with baseline stylization methods}. Our method produces spatially and temporally consistent style transfer results that faithfully match the style examples while maintaining photorealism. }
\label{fig:stylization}
\end{figure*}

\paragraph{Recoloring.} 

We use the HSV color space for recoloring in all experiments. Given a group of modified color palettes $\bm{\mathcal{P}}'$, we calculate the difference between the original palettes $\bm{\mathcal{P}}$ and $\bm{\mathcal{P}}'$ in HSV, then directly apply the change to all points' soft color, i.e. $\bm{\mathcal{P}} + \bm{\delta}(\bm{x})$. 

We compare our model with the state-of-the-art NeRF-based recoloring method PosterNeRF~\cite{posterNeRF} on the Blender Dataset in Fig.~\ref{fig:posterNeRF}. Our model produces more photorealistic results with fewer artifacts, and requires fewer palette edits. 

We also compare our model with a state-of-the-art palette-based video recoloring model~\cite{du2021video} in Fig.~\ref{fig:video_recolor} and image recoloring models~\cite{RGBXY, FSCS} in Fig.~\ref{fig:recolor}. Since our model consists of color offsets and radiance functions that extend the palette color to basis, it requires fewer palettes to reconstruct the images than other methods, which improves usability and benefits the quality of recoloring results. Also, with the help of the scene geometry, our results are more plausible in 3D. Particularly, we show recoloring results on two different views in the Kitchen scene, where we set the same recoloring goal for each of them: changing the light on the excavator to purple. While the image-based methods failed to keep the other objects looking the same from the two views, our model is able to produce view-consistent results for the whole scene.

\paragraph{Photorealistic style transfer.} We can apply our decomposition model to achieve \emph{photorealistic} style transfer on the captured scenes. Given a style image, users may define a series of correspondences between the image pixels and 3D points, that our system uses to transform our palette-based bases to align the point colors to the pixel colors; more details in the supplementary. We compare our model with three state-of-the-art methods: UPST-NeRF~\cite{UPST-NeRF}, ARF~\cite{ARF} and image-based stylization with AdaIN~\cite{AdaIN} (Fig.~\ref{fig:stylization}). Our results are more photorealistic than ARF and AdaIN, and comparable with UPST-NeRF. However, UPST-NeRF takes much more time to train (tens of hours) than ours.

\paragraph{User study.} To better demonstrate the effectiveness of our model, we also conduct a user study on these two applications. The study was taken on the Amazon Mechanical Turk platform, where we dispatched 162 questions 30 times to the crowd (4860 in total), and received 4496 answers. In each question, the user watches images/videos generated from our model and another randomly selected baseline and was asked to decide which one is more view-consistent and/or photorealistic. Fig.~\ref{fig:user_study} summarizes our study's results. We outperform image-based recoloring baselines~\cite{RGBXY, FSCS}, and are considered more photorealistic than  posterNeRF~\cite{posterNeRF}. For the style transfer task, our model received better feedback than ARF~\cite{ARF} and AdaIN~\cite{AdaIN} and is rated better than UPST-NeRF~\cite{UPST-NeRF} for view-consistency. More details are in the supplementary.

\subsection{Ablations}

We conduct two ablative evaluations on the LLFF dataset  to show the effectiveness of our model design. We first compare our model with the original vanilla Instant-NGP with two metrics: the Peak Signal-to-Noise Ratio (PSNR $\uparrow$), the Learned Perceptual Image Patch Similarity~\cite{LPIPS} (LPIPS$\downarrow$). Our model achieves the same PSNR score from the Instant-NGP (24.50), and has slightly higher LPIPS score (0.152 comparing to 0.145). This shows our model has little effect on the reconstruction quality. We then compare our model with three variants: Model without color offset (Ours w/o $\bm\delta$), model without the sparsity loss (Ours w/o $\mathcal{L}_\textbf{sp}$) and model without the smooth loss (Ours w/o $\mathcal{L}_\textbf{sm}$) both quantitatively and qualitatively. Quantitative results are shown in Tab.~\ref{tab:ablation}, where our full model achieves the best sparsity score among all models. Additionally, removing color offset will also decrease the quality of reconstruction in a perceptual way (LPIPS raises from 0.152 to 0.160). We also qualitatively shows comparisons in Fig.~\ref{fig:qualitative_ablation}, where removing smoothness loss leads to major artifacts in recoloring, and removing the sparsity loss results in color bleeding on unrelated areas (walls in the shown case). 

% Our ablative evaluation aims to show the effectiveness of our model design. We compare our model with four variants and the original vanilla Instant-NGP with four metrics: the Peak Signal-to-Noise Ratio (PSNR), the Learned Perceptual Image Patch Similarity~\cite{LPIPS} (LPIPS), the sparsity error defined by Eq.~\ref{eq:sparse_loss} and the total variation of the basis weight images (TV) which measures their smoothness. Results are shown in Tab.~\ref{tab:ablation}. In addition, we also qualitatively compare our model with all variants on the Fern data in Fig.~\ref{fig:qualitative_ablation}. While our model produces comparable reconstruction results as the original Instant-NGP, removing the color offset function reduces the perceptual quality of the results. Removing smoothness loss leads to major artifacts in recoloring, and removing the sparsity loss results in color bleeding on unrelated areas (walls in the shown case). Moreover, all of these variants generate less sparse segmentation than our full model does.

% and the second one explores the most proper dimension number of our compressed CLIP feature. 
% \zhengfei{first ablation: PSNR/SSIM/LPIPS/Sparsity/Smoothness, compare with NeRF, Model w/o sparsity, Model w/o Smoothness, modeh w/o Soft Palettes. also show a qualitative result on Fern}

% \begin{table}[h]
% \begin{center}
% \caption{\textbf{Ablation Study}. We show PSNR, LPIPS, Total Variance and Sparsity scores on our models.
% From top to bottom: Original NeRF; full model; model trained without color offset; model trained without view-depended basis; model trained without sparsity loss; model trained without smoothness loss. }

% \label{tab:ablation_1}
% \begin{tabular}{cc}
% \includegraphics[width=0.25\textwidth]{figures/experiment/6_ablation.pdf}
% &
% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
% %\vspace{-5px}
% {\small
% \begin{tabular}{P{32pt}P{30pt}P{32pt}}
% Methods & PSNR $\uparrow$ & LPIPS $\downarrow$ \\
% \hline
% NeRF
% & 24.50 & \textbf{0.145} \\
% Ours 
% & 24.50 & 0.152 \\
% \hline\hline
% & TV  $\downarrow$ & SP $\downarrow$ \\
% \hline
% w/o $\delta$ 
% & 0.263 & 0.647 \\
% w/o sp 
% & \textbf{0.123} & 1.643 \\
% w/o sm 
% & 0.549 & 0.554 \\
% Ours &  0.303 & \textbf{0.478} \\
% \hline

% \end{tabular}}
% \end{tabular}
% \end{center}
% %\vspace{-10px}
% \end{table}

\begin{table}
\begin{center}
\caption{\textbf{Quantitative ablation study results}. We compare our model with variants on two metrics: The sparsity error defined by Eq.~\ref{eq:sparse_loss} and the total variation of the weight images (TV) which measures their smoothness.}

\label{tab:ablation}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\vspace{-5px}
{\small
\begin{tabular}{P{53pt}P{38pt}P{38pt}}
Methods & Sparsity $\downarrow$ & TV  $\downarrow$  \\
\hline
Ours 
& \textbf{0.478} & 0.303  \\
Ours w/o $\bm{\delta}$ 
& 0.647 & 0.263  \\
% Ours w/o $s$ 
% & 24.12 & 0.155 & 0.323 & 0.557 \\
Ours w/o $\mathcal{L}_{\textrm{sp}}$ 
& 1.643 &  \textbf{0.123}  \\
Ours w/o $\mathcal{L}_{\textrm{sm}}$  
& 0.554 & 0.549  \\
\hline

\end{tabular}}
\end{center}
\vspace{-10px}
\end{table}

% \begin{table}
% \begin{center}
% \caption{\textbf{Quantitative ablation study results}. Top to bottom: Instant-NGP; full model; model trained w/o color offset; model trained w/o sparsity loss; model trained w/o smoothness loss. }

% \label{tab:ablation}
% \newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
% \vspace{-5px}
% {\small
% \begin{tabular}{P{53pt}P{31pt}P{31pt}P{25pt}P{38pt}}
% Methods & PSNR $\uparrow$ & LPIPS $\downarrow$ & TV  $\downarrow$ & Sparsity $\downarrow$ \\
% \hline
% Instant-NGP
% & 24.50 & \textbf{0.145} & - & - \\
% Ours 
% & 24.50 & 0.152 & 0.303 & \textbf{0.478} \\
% \hline
% Ours w/o $\bm{\delta}$ 
% & 24.46 & 0.160 & 0.263 & 0.647 \\
% % Ours w/o $s$ 
% % & 24.12 & 0.155 & 0.323 & 0.557 \\
% Ours w/o $\mathcal{L}_{\textrm{sp}}$ 
% & \textbf{24.51} & 0.152 & \textbf{0.123} & 1.643 \\
% Ours w/o $\mathcal{L}_{\textrm{sm}}$  
% & 24.50 & 0.152 & 0.549 & 0.554 \\
% \hline

% \end{tabular}}
% \end{center}
% \vspace{-10px}
% \end{table}

\begin{figure*}
\centering
\includegraphics[width=0.99\textwidth]{figures/experiment/6_ablation_v2.pdf}
\caption{\textbf{Qualitative ablation study results}. In this example we change the green palette (primarily representing the plants) to red color. }

\label{fig:qualitative_ablation}
\vspace{-5px}
\end{figure*}

% \begin{figure}
% \centering
% \includegraphics[width=0.48\textwidth]{figures/experiment/ablation_feature.pdf}
% \caption{Ablation Study on CLIP Feature. \zhengfei{Typo. Out of Memory}}
% \label{fig:ablation_feature}
% \end{figure}


\subsection{More Results}

In Fig.~\ref{fig:CLIPediting}, we show several results of feature-guided editing. Although our optimized segmentations are shared across the scene and do not directly support local editing, adding semantic features effectively resolves this issue.

\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/experiment/5_CLIP.pdf}
\caption{\textbf{Semantic guided editing}. On the left we show the unedited image and recolored results w/o feature guidance. On the right side, we show four guided results where individual objects (plant, floor, table, carpet) are exclusively edited.}
\label{fig:CLIPediting}
\vspace{-15pt}
\end{figure}

In Fig.~\ref{fig:application}, we show two more edits supported by our decomposition results. By scaling the view-dependent color function $\bm{s}(\bm{x}, \bm{d})$ and the color offset functions $\bm{\delta}_i(\bm{x})$, we can modify the illumination conditions and object textures of the scene, while keeping the rendering photorealistic.
\begin{figure}
\centering
\includegraphics[width=\linewidth]{figures/experiment/4_illumination.pdf}
\caption{\textbf{Additional appearance editing results.} \textit{First Row}: Rendered images with scaled view-dependent function; \textit{Second Row}: Rendered images with scaled color offset functions.}
\label{fig:application}
\end{figure}

==> (Arxiv) CVPR 2023 editing on NeRF with neural basis decomposition/sections/teaser.tex <==
% \begin{strip}\centering
% \includegraphics[width=\textwidth]{figures/teaser_v2.pdf}
% \captionof{figure}{We propose PaletteNeRF, a novel method for efficient appearance editing of neural radiance fields (NeRF). Taking (a) multi-view photos as training input, our approach reconstructs a NeRF and decomposes its appearance into (b) a set of color palettes and 3D-aware and view-consistent soft color segmentations through optimization, which enables (c) intuitive and photorealistic recoloring of the scene with 3D consistency across different views. Further, we show that (d) our method supports various palette-based appearance editing applications such as illumination modification and 3D photo-realistic style transfer.  
% \sai{Here the color pallets should be in 3D, but now we are showing it in 2D. I think it may cause some confusions. Some explanations are needed. At least it should be clearly annotated that (b) corresponds to the middle view in (a). Adding image borders to each image in (b). The stylization also looks suspicious to me.
% }
% \label{fig:teaser}}
% \end{strip}

\begin{strip}\centering
\vspace{-50px}
\includegraphics[width=\textwidth]{figures/teaser_v3.pdf}
\vspace{-10px}
\captionof{figure}{We propose \PaletteNeRF, a novel method for efficient appearance editing of neural radiance fields (NeRF). Taking (a) multi-view photos as training input, our approach reconstructs a NeRF and decomposes its appearance into a set of (b) 3D palette-based color bases. This enables (c) intuitive and photorealistic recoloring of the scene with 3D consistency across arbitrary views. Further, we show that (d) our method supports various palette-based editing applications such as illumination modification and 3D photorealistic style transfer.  
\label{fig:teaser}}
\end{strip}
